Online Trajectory Replanner for Dynamically Grasping Irregular Objects

This paper presents a new trajectory replanner for grasping irregular objects. Unlike conventional grasping tasks where the object's geometry is assumed simple, we aim to achieve a "dynamic grasp" of the irregular objects, which requires continuous adjustment during the grasping process. To effectively handle irregular objects, we propose a trajectory optimization framework that comprises two phases. Firstly, in a specified time limit of 10s, initial offline trajectories are computed for a seamless motion from an initial configuration of the robot to grasp the object and deliver it to a pre-defined target location. Secondly, fast online trajectory optimization is implemented to update robot trajectories in real-time within 100 ms. This helps to mitigate pose estimation errors from the vision system. To account for model inaccuracies, disturbances, and other non-modeled effects, trajectory tracking controllers for both the robot and the gripper are implemented to execute the optimal trajectories from the proposed framework. The intensive experimental results effectively demonstrate the performance of our trajectory planning framework in both simulation and real-world scenarios.

==> controllers.tex <==
\label{section: controller}
%To follow the desired trajectories presented in the previous 
%In addition, the robot has subordinate control based on singular perturbation theory and friction compensation. 
%The \ref{section: SDH2 controller} section deals with the design of the finger joint trajectory follower controller. 
%Given the internal control \ref{section: SDH2 controller} of the gripping hand, the trajectory follower controller is designed based on a two-degree-of-freedom control loop structure. 
%The guidance signal for the internal controller of the gripping hand is the desired velocity $\dot{\vec{q}}_{h,d}$ of the finger joints. By choosing a two-degree-of-freedom control loop structure, any deviations between the desired $\vec{q}_{h,d}$ and the actual $\vec{q}_{h}$ states are accounted for but compensated for. 
First, a trajectory tracking controller is presented for the gripper \schunk which is activated during the grasping process, %i.e. the red region in Fig. \ref{fig: timeline}. 
Subsequently, a computed-torque controller is introduced that enforces the robot to follow the desired trajectories $\bm{\xi}_i,\: i\in\{1,2,3\}$.

\subsection{Gripper controller}
\label{section: SDH2 controller}
%The Schunk gripper hand is connected to the PC via another network card. For the control and regulation according to section \ref{ch:controllers_hand} another \MatlabSimulink model was created, which runs independently from the robot in its own TwinCAT RT environment with a cycle time of $\SI{20}{\milli\second}$. A TwinCAT C/C++ module was programmed, which is responsible for the cyclic data exchange of the internal control of the gripping hand and the \MatlabSimulink model via Real-Time Ethernet. In the \MatlabSimulink model, one of the available internal controllers of the gripping hand (see chapter \ref{ch:controllers_hand}) can be preselected manually. 
%A position controller with constant maximum velocity $|\dot{\vec{q}}_h|=\dot{\vec{q}}_{h,max}$ and constant maximum acceleration $|\ddot{\vec{q}}_h|=\ddot{\vec{q}}_{h,max}$ is available for selection. Furthermore, two different speed controllers $\dot{\vec{q}}_h$, with maximum acceleration $|\ddot{\vec{q}}_h|=\ddot{\vec{q}}_{h,max}$ but with predetermined acceleration $|\dot{\vec{q}}_h|$ of the finger joints, can be selected. 
%Depending on the selected controller, different control commands are sent to the gripping hand. Depending on the controller selection, the created C/C++ module sends the required commands, reads the internal states of the hand and forwards them to the \MatlabSimulink model. 
%In addition, the \MatlabSimulink model includes the calculation of the target trajectory (\ref{eq:traj_hand_total}) and the trajectory follower controller from section \ref{ch:controllers_hand}. 
%The runtime $t$ of the experiment is read from the \MatlabSimulink model of the robot. 
%For performance reasons, the control commands can be sent to the gripping hand at most $\SI{50}{\hertz}$. 
%The gripping hand is equipped with pressure-sensitive surfaces, but these were not evaluated in this work. More detailed information about the possible settings can be found in the manual \cite{sdh2_manual}. 
%In the following section, a trajectory follower controller for the finger joints of the gripping hand is designed. 
Since the gripper has an internal controller from its manufacturer, it is not possible to directly specify the torques of the finger joints. There are three modes that can be chosen in the internal controller of the gripper listed in the following
\begin{itemize}
    \item \textit{Mode 1}: The position controller with the desired position input $\vec{q}_\hsym^*$. In this mode, the maximum velocity vector $\overline{\dot{\vec{q}}_{\hsym}}$ and the maximum acceleration $\overline{\ddot{\vec{q}}_{\hsym}}$ vector are predefined by the manufacturer.
    \item \textit{Mode 2}: The speed controller with the desired position input $\dot{\vec{q}}_\hsym^*$. In this mode, the maximum acceleration vector $\overline{\ddot{\vec{q}}_{\hsym}}$ is predefined by the manufacturer.
    \item \textit{Mode 3}: The speed controller with the desired position input $\dot{\vec{q}}_\hsym^*$ In this mode, the maximum acceleration $\overline{\ddot{\vec{q}}_{\hsym}}$ can be given as an additional input.
\end{itemize}
    
%More details about the hand configuration follow in chapter \ref{ch:implementation_results}.
%The internal controller chosen is the velocity controller for $\dot{\vec{q}}_h$ with a constant internal acceleration $\abs{\ddot{\vec{q}}_h}=\ddot{\vec{q}}_{h,max}$. 
In this work, mode 2 is chosen as the low-level control for the gripper. Since this mode only considers the desired velocity $\dot{\vec{q}}_{\hsym}^*$, deviations between the desired $\vec{q}_{\hsym}^*$ obtained from and the actual $\vec{q}_{\hsym}$ states may occur. 
Thus, a control scheme is implemented, shown in Figure \ref{fig:gripper_controller_schematics}. 
The desired set points for the internal speed controller $\dot{\vec{q}}_{\hsym,s}$ is formed by the sum of the optimal gripper state $\dot{\vec{q}}_{\hsym}^*$ and from a PI-controller, corresponding to
\begin{equation}
	\dot{\vec{q}}_{\hsym,s} = \dot{\vec{q}}_{\hsym}^*+\dot{\vec{q}}_{\hsym,e} \Comma
\end{equation}
where $\dot{\vec{q}}_{\hsym,e}$ is computed from
\begin{equation}
    \begin{aligned}
        \dot{\vec{q}}_{\hsym,e}&=\vec{K}_P\vec{q}_{\hsym,e}+\vec{K}_I\int_{}^{}\vec{q}_{\hsym,e}\text{d}t, \\
         \vec{q}_{\hsym,e}&=\vec{q}_{\hsym}^*-\vec{q}_{\hsym} \Comma
     \end{aligned}
\end{equation}
with the user-defined diagonal matrices $\vec{K}_P$ and $\vec{K}_I$. %The chosen values for $\vec{K}_P$ and $\vec{K}_I$ can be found in the table \ref{tab:controller_hand_params}.
\begin{figure}
    \centering
    \def\svgwidth{1\columnwidth}
    \input{./graphics/gripper_controller_schematics.pdf_tex}
    %\includegraphics[width=0.3\textwidth]{./iiwa_render/iiwa_render_crop.png}
    %\includegraphics[width = \columnwidth]{./figure/rotate_box.pdf_tex}
    \caption{Control structure of the gripper \schunk.}%
    \label{fig:gripper_controller_schematics}%
\end{figure}
\subsection{Computed torque controller for the robot motion}
\label{section: robot controller}
With the proposed computed torque controller, the robot follows the desired trajectory $\bm{\xi}^*(t)$. 
Since $\bm{\xi}^*(t)$ is twofold continuously differentiable, the computed torque controller reads as
\begin{equation}
\begin{aligned}
    \bm{\tau} &= \mathbf{C}(\mathbf{q},\dot{\mathbf{q}})\dot{\mathbf{q}} + \mathbf{g}(\mathbf{q}) +\mathbf{M}(\mathbf{q})(\mathbf{v}^*(t) - \mathbf{K}_2\dot{\mathbf{e}}_q-\mathbf{K}_{1}\mathbf{e}_q) \Comma
\end{aligned}
\end{equation}
where the trajectory errors are $\mathbf{e}_q=\mathbf{q}-\mathbf{q}^*((t))$ and $\dot{\mathbf{e}}_q=\dot{\mathbf{q}}-\dot{\mathbf{q}}^*(t)$. The user-defined positive definite control matrices are $\mathbf{K}_1 = \mathrm{diag}(k_{1,1},k_{1,2},...,k_{1,7})$ and $\mathbf{K}_2 = \mathrm{diag}(k_{2,1},k_{2,2},...,k_{2,7})$. 
Using a standard pole placement procedure \cite{spong2005robot}, the matrices $\mathbf{K}_1$ and $\mathbf{K}_2$ are chosen for this closed-loop control to be asymptotically stable. 
%For the trajectory follower of the robot, the control law of inverse dynamics or computed-torque with integral part \cite{siciliano}
%\begin{equation}
%\vec{\tau}_d=\vec{D}\left(\vec{q}\right)\vec{v}+\vec{C}\left(\vec{q},\dot{\vec{q}}\right)\dot{\vec{q}}+\vec{g}\left(\vec{q}\right)
%\end{equation}
%is used with the new place input $\vec{v}$. As explained in chapter \ref{ch:trajectories}, the influence of the Coriolis matrix is small and thus neglected. Accordingly, the given torque is calculated by
%\begin{equation}
%	\vec{\tau}_d=\vec{D}\left(\vec{q}\right)\vec{v}+\vec{g}\left(\vec{q}\right),
%\end{equation}
%where $\vec{v}$ denotes the new place input. The control input $\vec{v}$ now allows the formulation of the trajectory follower in the form
%\begin{equation}
%	\vec{v}=\ddot{\vec{q}}_d-\vec{K}_1\left(\dot{\vec{q}}-\dot{\vec{q}}_d\right)-\vec{K}_0\left(\vec{q}-\vec{q}_d\right)-\vec{K}_I\int_{}^{} \vec{q}-\vec{q}_d\text{d}t
%\end{equation}
%with the desired trajectory $\vec{q}_d$, $\dot{\vec{q}}_d$ and $\ddot{\vec{q}}_d\left(t\right)=\vec{u}\left(t\right)$ from (\ref{eq: traj_robot_total}), and the positive definite diagonal matrices $\vec{K}_0$, $\vec{K}_1$ and $\vec{K}_I$. It can be easily shown that the closed loop is asymptotically stable.




==> experimental_setup_modeling.tex <==
 \graphicspath{{./}{graphics/}}
 \label{sec: modeling}

In this section, the modeling of the robot and the \schunk (SDH2) gripper are briefly presented. 

%The \kuka is controlled by the PC via EtherCAT using the singular perturbation controller \cite{Ott2008}. 

%The provided \MatlabSimulink model was extended with the Kalman filter from Section \ref{chapter: object detection} and the trajectory optimization in Section \ref{chapter: trajectory optimizaton}. 


%The Schunk gripper hand is connected to the PC via another network card. 
%For the control and regulation according to section \ref{ch:controllers_hand}, another \MatlabSimulink model was created, which runs independently of the robot in its own TwinCAT RT environment with a cycle time of $\SI{20}{\milli\second}$. 
%A TwinCAT C/C++ module was programmed, which is responsible for the cyclic data exchange of the internal control of the gripping hand and the \MatlabSimulink model via Real-Time Ethernet. 
%In the \MatlabSimulink model, one of the available internal controllers of the gripping hand (see chapter \ref{ch:controllers_hand}) can be preselected manually. 
%A position controller with constant maximum velocity $|\dot{\vec{q}}_h|=\dot{\vec{q}}_{h,max}$ and constant maximum acceleration $|\ddot{\vec{q}}_h|=\ddot{\vec{q}}_{h,max}$ is available for selection. 
%Furthermore, two different speed controllers $\dot{\mathbf{q}}_h$, with maximum acceleration $|\ddot{\mathbf{q}}_h|=\ddot{\mathbf{q}}_{h,max}$ however with predetermined acceleration $|\dot{\vec{q}}_h|$ of the finger joints, can be selected. Depending on the selected controller, different control commands are sent to the gripping hand. Depending on the controller selection, the created C/C++ module sends the required commands, reads the internal states of the hand, and forwards them to the \MatlabSimulink model. 
%In addition, the \MatlabSimulink model includes the calculation of the target trajectory (\ref{eq:traj_hand_total}) and the trajectory follower controller from section \ref{ch:controllers_hand}. 
%The runtime $t$ of the experiment is read from the \MatlabSimulink model of the robot. 
%For performance reasons, the control commands can be sent to the gripping hand at most $\SI{50}{\hertz}$. 
%The gripping hand is equipped with pressure-sensitive surfaces, but these were not evaluated in this work. 
%More detailed information about the possible settings can be found in the manual \cite{sdh2_manual}. 

%The camera is connected to the PC via Gigabit. For reading the images the Python module pypylon is used \cite{pypylon}, which is provided by Basler. 
%The images are read out cyclically in a Python script. 
%For image processing, detecting the ArUco markers, extracting the point matrix $\bar{\vec{p}}$ and computing (\ref{eq:EPnP}) the respective implementations of the freely available library OpenCV version 4.2 including the extra modules \cite{opencv_lib, opencv_contrib_lib} are used. 
%In each image, the ArUco markers are detected, and the pose of the coordinate system \kos{o} with respect to the camera \kos{c} is computed and passed to the Kalman filter in the robot model via the ADS library \cite{pyads}.
\subsection{Modeling of the \kuka robot}
%\subsubsection{The \kuka robot}
\begin{figure}
    \centering
    \def\svgwidth{1\columnwidth}
    \input{./graphics/system_schematics.pdf_tex}
    %\includegraphics[width=0.3\textwidth]{./iiwa_render/iiwa_render_crop.png}
    %\includegraphics[width = \columnwidth]{./figure/rotate_box.pdf_tex}
    \caption{Schematic drawing of (a) the \kuka, (b) the \schunk (SDH 2), (c) the camera \camera, and (d) the object. The $x$-, $y$-, and $z$-axis of each coordinate frame are shown as red, green, and blue arrows, respectively. In the tuple of the rotation angle
    and its corresponding coordinate frame $(\mathcal{O}_{\hsym,i},q_{\hsym,i})$, the illustrating color of the joint angle $q_{\hsym,i}$ matches the corresponding rotate axis.}%
    \label{fig: schematics}%
\end{figure}
The robot is modeled as a rigid-body system with the generalized coordinates $\mathbf{q}^\mathrm{T} = [q_1,q_2,\dots,q_7]$, see Fig. \ref{fig: schematics}(a), which are the rotation angles $q_i$ around the $z$-axes (blue arrows) of each coordinate frame $\mathcal{O}_i$, $i=1,\dots,7$. 
To describe the kinematic relationship between the joint angles and the pose of the robot links comprising position and orientation, the homogeneous transformations $\mathbf{H}_n^m$ between two adjacent frames $\mathcal{O}_n$ and $\mathcal{O}_m$ are constructed, see Tab. \ref{table: coordinate transformation}.
Here and in the following, the homogeneous transformation of a simple translation by distance $d$ along the local axis $j \in \{x, y,z\}$ is denoted by $\mathbf{H}_{\mathbf{D},j}(d)$, while an elementary rotation around the local axis $j \in \{x,y,z\}$ by the angle $\phi$ is described by $\mathbf{H}_{\mathbf{R},j}(\phi)$. 

\begin{table}
	\begin{center}%[table-unit-alignment=left]
		\begin{tabular}{c c c}
                \hline 
			  \makecell{Frame \\$\mathcal{O}_n$}& \makecell{Frame\\ $\mathcal{O}_m$} & \makecell{\textbf{Transformation matrix} \\$\mathbf{H}_{i}^{j}$}\\
                %\hline
                \hline  \noalign{\vskip 0.05cm}    
   			0 & 1 & $\mathbf{H}_{\mathbf{D},z}(d_1) \mathbf{H}_{\mathbf{R},z}(q_1)$\\
			1 & 2 & $\mathbf{H}_{\mathbf{D},z}(d_2)\mathbf{H}_{\mathbf{R},z}(-\pi)\mathbf{H}_{\mathbf{R},x}(\pi/2)\mathbf{H}_{\mathbf{R},z}(q_2)$ \\
			2 & 3 & $\mathbf{H}_{\mathbf{D},y}(d_3)\mathbf{H}_{\mathbf{R},z}(\pi)\mathbf{H}_{\mathbf{R},x}(\pi/2)\mathbf{R}_z(q_3)$\\
			3 & 4 & $\mathbf{H}_{\mathbf{H},z}(d_4) \mathbf{H}_{\mathbf{R},x}(\pi/2)\mathbf{H}_{\mathbf{R},z}(q_4)$\\
			4 & 5 & $\mathbf{H}_{\mathbf{D},y}(d_5) \mathbf{H}_{\mathbf{R},z}(\pi)\mathbf{H}_{\mathbf{R},x}(\pi/2)\mathbf{H}_{\mathbf{R},z}(q_5)$\\
			5 & 6 & $\mathbf{H}_{\mathbf{D},y}(d_6) \mathbf{H}_{\mathbf{R},x}(\pi/2)\mathbf{H}_{\mathbf{R},z}(q_6)$\\
			6 & 7 & $\mathbf{H}_{\mathbf{D},z}(d_7) \mathbf{H}_{\mathbf{R},z}(\pi)\mathbf{H}_{\mathbf{R},x}(\pi/2)\mathbf{H}_{\mathbf{R},z}(q_7)$\\
			7 & $\esym$ & $\mathbf{H}_{\mathbf{D},z}(d_e)$\\
                7 & $\csym$ & $\mathbf{H}_{\mathbf{D},y}(l_c)\mathbf{H}_{\mathbf{D},z}(d_c) \mathbf{H}_{\mathbf{R},z}(\pi)\mathbf{H}_{\mathbf{R},x}(\theta_c)$\\
                7 & $\hsym$ & $\mathbf{H}_{\mathbf{D},z}(d_h) \mathbf{H}_{\mathbf{R},z}(\pi/2)$\\
                \hline
		\end{tabular}
	\end{center}
	\caption{Translation and rotation from the coordinate systems $\mathcal{O}_m$ and  $\mathcal{O}_n$ for the robot system with the gripper.}
	\label{table: coordinate transformation}
\end{table}


\begin{table}
\caption{Kinematic and dynamic limits of the \kuka}
\label{table: constraints}
\begin{center}
\scalebox{1}{
\begin{tabular}{c c c c c }
%\hline
\textbf{Joint} $i$ & \textbf{Joint limits} & \textbf{Velocity limits} & \textbf{Torque limits} \\
 & $\overline{q_i}$ ($^{\circ}$) & $\overline{\dot{q}_i}$ ($^{\circ}$/\SI{}{\second}) & $\overline{\tau_{i}}$ (\SI{}{\newton}) \\
\hline
1 & 170 & 85 & 320 \\
%\hline
2 & 120 & 85 & 320 \\
%\hline
3 & 170 & 100 & 176 \\
%\hline
4 & 120 & 75 & 176 \\
%\hline
5 & 170 & 130 & 110 \\
%\hline
6 & 120 & 135 & 40 \\
%\hline
7 & 175 & 135 & 40 \\
\hline
\end{tabular}
}
\end{center}
\end{table}

The end-effector transformation matrix $\mathbf{H}_0^\esym$ is referred to as forward kinematics and is computed in the form
\begin{equation}
\mathbf{H}_0^\esym = \mathrm{FK}(\mathbf{q}) =\left(\prod_{i=0}^{7}\mathbf{H}_{i}^{i+1}\right)\mathbf{H}^\esym_7 = \begin{bmatrix}
\mathbf{R}_0^\esym(\mathbf{q}) & \mathbf{p}_\esym(\mathbf{q}) \\
\mathbf{0} & \mathbf{1}
\end{bmatrix} \Comma
\label{eq: FK}
\end{equation}
comprising the Cartesian position $\mathbf{p}_\esym \in \mathbb{R}^3$ and the rotation matrix $\mathbf{R}_0^\esym \in \mathrm{SO(3)}$. 
Similarly, the homogeneous transformations from the world frame $\mathcal{O}_0$ to the SDH2 and the camera frame read as
\begin{subequations}\label{eq: FK hand and camera}

    \begin{align}
        \label{eq: FK hand}
        \mathbf{H}_0^\hsym &= \left(\prod_{i=0}^{7}\mathbf{H}_{i}^{i+1}\right)\mathbf{H}^\hsym_7 = \begin{bmatrix}
\mathbf{R}_0^\hsym(\mathbf{q}) & \mathbf{p}_0^\hsym(\mathbf{q}) \\
\mathbf{0} & \mathbf{1}
\end{bmatrix} \Comma \\
       \label{eq: FK camera}
         \mathbf{H}_0^\csym &= \left(\prod_{i=0}^{7}\mathbf{H}_{i}^{i+1}\right)\mathbf{H}^\csym_7 = \begin{bmatrix}
\mathbf{R}_0^\csym(\mathbf{q}) & \mathbf{p}_0^\csym(\mathbf{q}) \\
\mathbf{0} & \mathbf{1}
\end{bmatrix} \FullStop 
    \end{align}
    
\end{subequations}

The equations of motion are derived using the Lagrange formalism, see, e.g., \cite{spong2005robot}, 
\begin{equation}
\mathbf{M}(\mathbf{q})\ddot{\mathbf{q}} + \mathbf{C}(\mathbf{q},\dot{\mathbf{q}})\dot{\mathbf{q}} + \mathbf{g}(\mathbf{q}) = 
\bm{\tau},
\label{eq: EOM}
\end{equation}
where $\mathbf{M}(\mathbf{q})$ denotes the symmetric and positive definite mass matrix, $\mathbf{C}(\mathbf{q}, \dot{\mathbf{q}})$ is the Coriolis matrix, $\mathbf{g}(\mathbf{q})$ is the force vector associated with the potential energy, and $\bm{\tau}$ are the motor torque inputs. Note that friction and elastic joints are neglected here for brevity. A full elastic joint model can be found in, e.g.,~\cite{Ott2008}.
%The kinematic and dynamic parameters of the KUKA LBR iiwa in (\ref{eq: EOM}) are taken from \cite{sturz2017parameter}. 
Since the mass matrix $\mathbf{M}(\mathbf{q})$ is invertible, (\ref{eq: EOM}) is rewritten in the state-space form 
\begin{equation}
\dot{\mathbf{x}} = 
\begin{bmatrix}
\dot{\mathbf{q}} \\
\mathbf{M}^{-1}(\mathbf{q}) (\bm{\tau}-\mathbf{C}(\mathbf{q},\dot{\mathbf{q}})\dot{\mathbf{q}}-\mathbf{g}(\mathbf{q}))
\end{bmatrix},
\label{eq: state space}
\end{equation} 
with the system state $\mathbf{x}^{\mathrm{T}} = [\mathbf{q}^{\mathrm{T}},\dot{\mathbf{q}}^{\mathrm{T}}]$. 
The kinematic and dynamic limits of the robot \cite{kukalbriiwa} are summarized in Tab. \ref{table: constraints}. All limits are symmetric w.r.t. zero, i.e. $\underline{q_i} = -\overline{q_i}$, $\underline{\dot{q}_i} = -\overline{\dot{q}_i}$, and $\underline{\tau_{i}} = -\overline{\tau_{i}}$.

It is assumed that the nonlinear dynamics are compensated by an inverse dynamics control law of the form
\begin{align}
  \label{eqn:computed_torque}
  \vect{\tau} = \vect{M}(\vect{q})\vect{v} + \vect{C}(\vect{q}, \dot{\vect{q}})\dot{\vect{q}} + \vect{g}(\vect{q})\Comma
\end{align}
resulting in the remaining linear dynamics
\begin{align}
  \label{eqn:double_integrator}
  \ddot{\vect{q}} = \vect{v}\Comma
\end{align}
with the virtual input $\vect{v}$. 
Note the state-space form of this remaining linear dynamics is expressed as
\begin{equation}
    \dot{\mathbf{x}} = \mathbf{f}(\mathbf{x},\mathbf{v}) = [(\dot{\mathbf{q}})^\mathrm{T},\mathbf{v}^\mathrm{T}]^\mathrm{T}
    \label{eq: remaining dynamics state-space form}
\end{equation}

%Different approaches exist for stabilizing the linear system including Cartesian impedance control. 
%In the following, a reference trajectory is planned for the remaining linear dynamics. 
\subsection{Modeling of \schunk gripper}
%\subsubsection{The gripper (SDH 2)} 
\begin{figure}
    \centering
    \def\svgwidth{1\columnwidth}
    \input{./graphics/SHD2_schematics.pdf_tex}
    %\includegraphics[width=0.3\textwidth]{./iiwa_render/iiwa_render_crop.png}
    %\includegraphics[width = \columnwidth]{./figure/rotate_box.pdf_tex}
    \caption{(a) Side view of the SDH2 without the finger 2 with $q_{\hsym,1}=-q_{\hsym,6}=-\pi/2$. (b) Side view of the gripping hand with the SDH2 state variables $\vec{q}_\hsym$ and the grasping state $\vec{q}_G$.}%
    \label{fig: SDH2 schematics}%
\end{figure}
The SDH2, attached to the robot end effector, consists of three fingers shown in Fig. \ref{fig: schematics}(b).
Each finger consists of a proximal and a distal phalanx, which is connected by a rotary joint. 
The proximal phalanx is connected to the base via another rotary joint, resulting in two degrees of freedom per finger. 
The additional DoF allows the rotation of finger 1, i.e. $q_{\hsym,1}$,  and finger 3, i.e. $q_{\hsym,6}$,  around the corresponding $z$-axis. 
Note that fingers 1 and 3 are operated synchronously, however, in opposite directions.
In this work, only fingers 1 and finger 3 are utilized for grasping the object. 
Thus, finger 2 remains at the initial configuration $q_{\hsym,4}=\pi/2$ \SI{}{\radian} and $q_{\hsym,5}=\pi/3$ \SI{}{\radian}.  
In addition, to simplify the grasping problem, fingers 2 and 3 are positioned in the facing direction with fixed angles $q_{\hsym,1}=-q_{\hsym,6}=-\pi/2$, see Fig. \ref{fig: SDH2 schematics}. Thus, the system state of the SDH2 consists of four DoF $\mathbf{q}_\hsym^\mathrm{T} = [q_{\hsym,2},q_{\hsym,3},q_{\hsym,7},q_{\hsym,8}]$, see Fig. \ref{fig: SDH2 schematics}(b). 

The grasping (contact) point $\mathrm{G}$ is chosen as the midpoint of the line between the points $\mathrm{C}_1$ and $\mathrm{C}_3$. 
These points are the centers of arcs formed by the tactile sensor surfaces of fingers 1 and 3, respectively. 
Note that the choice of this grasping point is very crucial to achieve the steady state movement of the object after grasping. 
This is because the contact points at the object's surface will be perpendicular to the arcs of tactile sensor surfaces. Thereby, the contact forces are equally distributed to the surface of the object. 
The forward kinematics formulation
\begin{equation}
    \vec{p}_{\hsym}^{\mathrm{G}}=[x_\mathrm{G},y_\mathrm{G},z_\mathrm{G}]^\mathrm{T} = \mathrm{SHD2\_FK}(\vec{q}_\hsym)
    \label{eq: SDH2 FK}
\end{equation}
describes the position of the grasping point $\mathrm{G}$ depending on the joint coordinates $\vec{q}_\hsym$. 

To grasp an object, the grasping state 
$\vec{q}_\mathrm{G}= \transpose{\left[d_\mathrm{G}, \varphi_\mathrm{G},y_\mathrm{G}, z_\mathrm{G}\right]}$ 
is considered, where $d_G$ is the distance between the tactile sensor arcs, $\varphi_G$ is the tilting angle around the $x$-axis of the hand frame $\mathcal{O}_\hsym$ w.r.t. the line between the points $\mathrm{C}_1$ and $\mathrm{C}_3$, see Fig. \ref{fig: SDH2 schematics}(b). $y_\mathrm{G}$ and $ z_\mathrm{G}$ are the two elements of the position $\vec{p}_{\hsym}^{\mathrm{G}}$ of the grasping point $\mathrm{G}$. Note that the element $x_G$ in $\vec{p}_{\hsym}^{\mathrm{G}}$ is neglected since it coincides with the position of the origin of the hand coordinate $\mathcal{O}_\hsym$ in $x$-direction.   
Thus, the inverse kinematics of the SDH2 is necessary to compute the hand state $\mathbf{q}_{\hsym}$ with the given grasping state in the following
\begin{equation}
    \mathbf{q}_{\hsym} = \mathrm{SDH2\_IK}(\mathbf{q}_\mathrm{G}) \FullStop
    \label{eq: SDH2 IK}
\end{equation}
%For more details on (\ref{eq: SDH2 FK}) and (\ref{eq: SDH2 IK}), readers are referred to the appendix in Section \ref{section: appendix}. 
%where the grasping state $\vec{q}_\mathrm{G}= \transpose{\left[d_\mathrm{G}, \varphi_\mathrm{G},y_\mathrm{G}, z_\mathrm{G}\right]}$ is introduced, see Fig. \ref{fig: SDH2 schematics}(b). . In the following, (\ref{eq: SDH2 inv}) is presented in detail. 

%\begin{align}
%y_{C1} & = y_G-\left(r_{T2}+\frac{d_G}{2}\right)\cos\left(\varphi_G\right), \\
%z_{C1} & = z_G-\left(r_{T2}+\frac{d_G}{2}\right)\sin\left(\varphi_G\right), \\
%y_{C3} & = y_G+\left(r_{T2}+\frac{d_G}{2}\right)\cos\left(\varphi_G\right), \\
%z_{C3} & = z_G+\left(r_{T2}+\frac{d_G}{2}\right)\sin\left(\varphi_G\right). 
%\end{align}




%For the planning of a grip, four new state variables $\vec{q}_G= \transpose{\left[d_G, \varphi_G,y_G, z_G\right]}$ are introduced by which the grip state is described. They are shown in \prettyref{fig:hand_kinematics}. Here $y_G$ and $z_G$ denote the $y$ and $z$ components of the grasping point $G$ with respect to the coordinate system $(0_{h}x_{h}y_{h}z_{h})$. $\varphi_G$ describes the grasping angle and $d_G$ defines how wide the fingers are open. In this section, we derive the inverse kinematics. This allows the state variables $q_{h2}$, $q_{h3}$, $q_{h6}$ and $q_{h7}$ to be calculated as a function of the state variables $\vec{q}_G$. For better readability, the arguments $\vec{q}_G$ are omitted in the remainder of this paper.


%The forward kinematics $\vec{p}_{\hsym}^{\mathrm{G}}\left(\vec{q}_\hsym\right)$ describes the position of the grasping point $\mathrm{G}$ depending on the joint coordinates $\vec{q}_\hsym$. 
%For better readability, the arguments $\vec{q}_h$ are omitted in the remainder of this section. 
%In this section the vector $\vec{p}_j^k$ denotes a translation and the matrix $\vec{R}_j^k$ a rotation between two coordinate systems \kos{j} and \kos{k}.





%The schematics The required parameters are plotted in Fig \ref{fig: SDH2 schematics}. 



==> graphics/iiwa.tex <==
\begin{lpic}[l(0\textwidth),r(0\textwidth),t(0\textwidth),b(0\textwidth)]{iiwa_all(0.25)}%
%\begin{lpic}[l(0\textwidth),r(0\textwidth),t(0\textwidth),b(0\textwidth),draft]{iiwa_all(0.25)}%

\centering

\lbl[]{30,0,0;\color{red}\scalebox{0.72}{$x_0$}}%
\lbl[]{12,15,0;\color{blue}\scalebox{0.72}{$z_0$}}%

\lbl[]{45,60,0;\color{red}\scalebox{0.72}{$x_1$,$x_2$}}%
\lbl[]{12,50,0;\color{blue}\scalebox{0.72}{$z_1$}}%
\lbl[]{12,70,0;\color{blue}\scalebox{0.72}{$z_2$}}%

\lbl[]{0,120,0;\color{red}\scalebox{0.72}{$x_3$,$x_4$}}%
\lbl[]{42,117,0;\color{blue}\scalebox{0.72}{$z_3$}}%
\lbl[]{12,135,0;\color{blue}\scalebox{0.72}{$z_4$}}%

\lbl[]{40,177,0;\color{red}\scalebox{0.72}{$x_5$}}%
\lbl[]{7,180,0;\color{blue}\scalebox{0.72}{$z_5$}}%

\lbl[]{42,192,0;\color{blue}\scalebox{0.72}{$z_6$,$z_7$}}%
\lbl[]{5,170,0;\color{red}\scalebox{0.72}{$x_6$,$x_7$}}%

\lbl[]{12,217,0;\color{blue}\scalebox{0.72}{$z_e$}}%

\lbl[]{-10,210,0;\color{black}\scalebox{0.72}{\textbf{(a)}}}%

\lbl[]{12,205,0;\color{red}\scalebox{0.72}{$x_e$}}%

\lbl[]{30,18,0;\color{black}\scalebox{0.72}{$q_1$}}%
\lbl[]{30,50,0;\color{black}\scalebox{0.72}{$q_2$}}%
\lbl[]{30,82,0;\color{black}\scalebox{0.72}{$q_3$}}%
\lbl[]{30,110,0;\color{black}\scalebox{0.72}{$q_4$}}%
\lbl[]{30,142,0;\color{black}\scalebox{0.72}{$q_5$}}%
\lbl[]{30,167,0;\color{black}\scalebox{0.72}{$q_6$}}%
\lbl[]{7,192,0;\color{black}\scalebox{0.72}{$q_7$}}%

\end{lpic}%

==> object_detection.tex <==
\label{chapter: object detection}
%In this section, the camera-based estimation of the pose of the object, see Fig. \ref{fig: schematics}(d), is presented. 
This grasped object is equipped with an ArUco marker at the origin of the object coordinate $\mathcal{O}_o$.
First, the determination of the object's pose $[\mathbf{R}_\csym^\osym|\mathbf{p}_\csym^\osym]$ in the object frame $\mathcal{O}_o$ w.r.t. the camera frame $\mathcal{O}_c$ is briefly presented. 
Subsequently, an extended Kalman filter (EKF) is implemented to smooth the estimated pose during the robot motion. 
%$[\mathbf{R}_c^o]$ 
%Section \ref{ch:pose_estimation_kamera} explains the determination of the pose using a camera image and ArUco markers. These are suitably placed at known positions of the object to be grasped.
%In order toin the second part.

\subsection{Object's pose estimation via an ArUco Marker}
The calibration parameters, i.e. the camera matrix and distortion coefficients,  of the camera \camera, are computed by using the open source library OpenCV \cite{kaehler2016learning}. 
The pose of the gripping object $ \left[\vec{R}_\csym^\osym|\vec{p}_\csym^\osym\right] $ is estimated with the help of an ArUco marker \cite{garrido2014automatic}, see Fig. \ref{fig: aruco marker}, which is attached at the origin of the frame $\mathcal{O}_o$. 

For each vertex $\:i\in\{1,..,4\}$ of the ArUco marker, the 3D position $\tilde{\mathbf{P}}_i$ in the camera frame $\mathcal{O}_c$ and the 2D pixel coordinate $\tilde{\mathbf{p}}_i$ in the image frame, are estimated using the ArUco module of the OpenCV library. 
%In addition, each marker is assigned a unique $ID$ by the different arrangement of the white squares inside. 
%Thus, for each of the four vertices of $n$ visible ArUco markers on an image, the point pairs $(\tilde{\vec{p}}_i,\tilde{\vec{P}}_i), i \in \left\{1,\dots,4n\right\}$ can be created. 
These estimations are then combined into the matrices $\bar{\vec{p}}=\transpose{\rbraces{\tilde{\vec{p}}_1, \dots, \tilde{\vec{p}}_{4}}}$ and $\bar{\vec{P}}=\transpose{\rbraces{\tilde{\vec{P}}_1, \dots,\tilde{\vec{P}}_{4}}}$. 
Thereby, together with the calibration parameters of the camera, the object pose with respect to the camera coordinate system is calculated via the  Efficient Perspective-n-Point (EP\textit{n}P) algorithm \cite{lepetit2009epnp} in the form
\begin{equation}\label{eq:EPnP}
	\left[\vec{R}_\csym^\osym|\vec{p}_\csym^\osym\right] = \text{EPnP}\left(\bar{\vec{p}},\bar{\vec{P}}\right)\FullStop
\end{equation}
\begin{figure}
    \centering
    \def\svgwidth{0.2\columnwidth}
    \input{./graphics/arUco_markers.pdf_tex}
    %\includegraphics[width=0.3\textwidth]{./iiwa_render/iiwa_render_crop.png}
    %\includegraphics[width = \columnwidth]{./figure/rotate_box.pdf_tex}
    \caption{ArUco Marker $ID=2$ \cite{garrido2014automatic}.}%
    \label{fig: aruco marker}%
\end{figure}
For more information on the ArUco marker and  the EP\textit{n}P algorithm, readers are referred to \cite{garrido2014automatic} and \cite{lepetit2009epnp}.
\subsection{Extended Kalman Filter}
\label{section: ekf}
%Machine vision applications are very computationally intensive. 
%Reading the image, identifying the ArUco markers, and calculating the pose takes quite a few milliseconds. 
Since the camera is located at the end effector, the estimated pose between consecutively captured images is altered due to the movement of the robot. 
%During the robot motion, based on the estimated pose of the object w.r.t. the camera frame $\mathcal{O}_c$, an online trajectory optimization of the robot is performed cyclically presented in the next section. 
%The start time of the trajectory update is independent of the pose estimation. 
%Note that the trajectory update frequency is not constant. 
%Thus, it is not defined at which times the estimated pose is used to calculate the trajectory update. 
To account for the robot's motion and thus improve the object's pose estimation, an Extended Kalman filter is implemented. 
%The state estimation is done based on the robot's motion and a measurement update is performed using the computed pose from the camera image. 

%To design the Extended Kalman filter, a nonlinear continuous-time system model for the rotation and distance between the object and the camera is first derived. 
%In the next step, this continuous-time model is transformed into a nonlinear sampling system via the Euler method, on the basis of which the Extended Kalman filter is finally designed. 
%The derivation of the system models and the design of the Extended Kalman filter is performed based on \cite{Koenigseder17}.

The rotation between the camera coordinate system $\mathcal{O}_c$ and the object coordinate system $\mathcal{O}_o$ is expressed via a unit quaternion in the form
\begin{equation}
	(\vec{r}_\csym^\osym)^\mathrm{T}=\begin{bmatrix}
		r_0,r_1,r_2,r_3
	\end{bmatrix} = \begin{bmatrix}
	r_0,\vec{r}_{1:3}
%\end{bmatrix}=\begin{bmatrix}
%	\cos\left(\frac{\alpha}{2}\right)\\
%\transpose{\vec{n}}\sin\left(\frac{\alpha}{2}\right)
\end{bmatrix}, \quad \norm{\vec{r}}_2=1 \FullStop
\label{eq: quaternion}
\end{equation}
The relation between the quaternion $\vec{r}_\csym^\osym$ and the rotation matrix $\mathbf{R}_\csym^\osym$, obtained from the EP\textit{n}P algorithm in (\ref{eq:EPnP}), can be computed analytically, see \cite{shepperd1978quaternion}. %The distance from the object frame \mathcal{} to the 
The time derivative of the quaternion $\vec{r}_\csym^\osym$ reads as
\begin{equation}
	\dot{\vec{r}}_\csym^\osym = \frac{1}{2}\vec{\Omega}(\bm{\omega}_\csym^\osym)\vec{r}_\csym^\osym
\end{equation}
where $(\bm{\omega}_\csym^\osym)^\mathrm{T} = \rbraces{\omega_{\csym,x}^\osym, \omega_{\csym,y}^\osym, \omega_{\csym,z}^\osym} $ is the angular velocity of the object frame $\mathcal{O}_o$ w.r.t. the camera frame $\mathcal{O}_c$ and $\bm{\Omega}(\bm{\omega}_\csym^\osym)$ is the skew-symmetric matrix of the vector $[0,(\bm{\omega}_\csym^\osym)^\mathrm{T}]^\mathrm{T}$ expressed in the form
\begin{equation}
	\vec{\Omega}(\bm{\omega}_\csym^\osym) = \begin{bmatrix}
		0 & -\omega_{\csym,x}^\osym & -\omega_{\csym,y}^\osym & -\omega_{\csym,z}^\osym\\
		\omega_{\csym,x}^\osym & 0 & \omega_{\csym,z}^\osym & -\omega_{\csym,y}^\osym\\
		\omega_{\csym,y}^\osym & -\omega_{\csym,z}^\osym & 0 & \omega_{\csym,x}^\osym\\
		\omega_{\csym,z}^\osym & \omega_{\csym,y}^\osym & -\omega_{\csym,x}^\osym & 0\\
	\end{bmatrix} \FullStop
\end{equation}
%To complete the pose of the object coordinate system $\mathcal{O}_o$ with respect to the camera coordinate system $\mathcal{O}_c$, the distance vector $\vec{d}_c^o$ and its time derivative $\dot{\vec{d}}_c^o$ are defined. The distance to the object in the base coordinate system results from the homogeneous transformation $\vec{H}_0^c$ (\ref{eq: homogeneous_transformation_camera}) and the constant, but undefined position vector $\vec{d}_0^o$ of the object with respect to the base coordinate system to $\vec{d}_c^o=-\vec{d}_0^c+\vec{d}_0^o$ with the time derivative $\dot{\vec{d}}_c^o=-\dot{\vec{d}}_c^o=-\vec{v}_c$.
The angular velocity $\bm{\omega}_\csym^\osym$ and the linear velocity $\dot{\vec{p}}_\csym^\osym$ are computed as 
\begin{equation}\label{eq:manipulator-jacobi_camera}
	\begin{bmatrix}
		\bm{\omega}_\csym^\osym\\
		\dot{\vec{p}}_\csym^\osym
	\end{bmatrix} =\begin{bmatrix}
		\tilde{\bm{\omega}}_\csym^\osym-\vec{w}_\omega\\
		\tilde{\dot{\vec{p}}}_\csym^\osym-\vec{w}_v
	\end{bmatrix} \Comma
    %=
    %\begin{bmatrix}
	%\transpose{\braces{\vec{R}_0^c}}\tilde{\vec{\omega}}_0^c-\vec{w}_\omega\\
	%\tilde{\vec{v}}_0^c-\vec{w}_v
    %\end{bmatrix}
\end{equation}
where the measured angular rate $\tilde{\bm{\omega}}_\csym^\osym$ can be taken from the skew-symmetric matrix 
\begin{equation}
\begin{aligned}
 [\tilde{\bm{\omega}}_\csym^\osym]_\times &= \dfrac{\mathrm{d}}{\mathrm{d}t}(\mathbf{R}_\csym^\osym)(\mathbf{R}_\csym^\osym)^\mathrm{T} = \dfrac{\mathrm{d}}{\mathrm{d}t}(\mathbf{R}_\csym^0\mathbf{R}_0^\osym)(\mathbf{R}_\csym^0\mathbf{R}_0^\osym)^\mathrm{T} \\
 & = \dfrac{\mathrm{d}}{\mathrm{d}t}(\mathbf{R}_\csym^0)(\mathbf{R}_\csym^0)^\mathrm{T} + (\mathbf{R}_0^\csym)^\mathrm{T}\dfrac{\mathrm{d}}{\mathrm{d}t}(\mathbf{R}_0^\osym)(\mathbf{R}_0^\osym)^\mathrm{T}\mathbf{R}_0^\csym \\
 & = [\tilde{\bm{\omega}}_\csym^0]_\times + (\mathbf{R}_0^\csym)^\mathrm{T}[\tilde{\bm{\omega}}_0^\osym]_\times\mathbf{R}_0^\csym \Comma
 \end{aligned}
 \label{eq: angular rate ekf}
\end{equation}
%\begin{equation}
% \end{equation}
the estimated linear velocity $\tilde{\dot{\mathbf{p}}}_\csym^\osym$ reads as 
\begin{equation}
    \tilde{\dot{\mathbf{p}}}_\csym^\osym = -\tilde{\dot{\mathbf{p}}}_0^\csym + \tilde{\dot{\mathbf{p}}}_0^\osym \Comma
 \label{eq: linear rate ekf}
\end{equation}
and $\vec{w}_\omega$ and $\vec{w}_v$ are stochastic perturbations. Note that $[\mathbf{a}]_\times$ denotes the skew-symmetric matrix of the vector $\mathbf{a}$.
%Note that the relation between the angular velocity $\bm{\omega}_\csym$ and the camera rotation matrix $\mathbf{R}_0^\csym$ is computed via
%\begin{equation}
%    \mathbf{S}(\bm{\omega}_\csym) = \dfrac{\mathrm{d}}{\mathrm{d}t}(\mathbf{R}_0^\csym)(\mathbf{R}_0^\csym)^\mathrm{T} = \begin{bmatrix}
%        0 & -\omega_{c,z} & \omega_{c,y} \\
%        \omega_{c,z} & 0 &-\omega_{c,x} \\
%        -\omega_{c,y} & \omega_{c,x} & 0
%    \end{bmatrix} \FullStop
%\end{equation}
Since the gripped object is considered to be fixed, i.e., $\tilde{\dot{\mathbf{p}}}_0^\osym = 0$ and  $[\tilde{\bm{\omega}}_0^\osym]_\times=0$, the measured values of the angular rate and the linear velocity in (\ref{eq: angular rate ekf}) and (\ref{eq: linear rate ekf}), respectively, are computed by using only (\ref{eq: FK camera}) with the measured joint angles $\mathbf{q}$ and joint velocities $\dot{\mathbf{q}}$ of the robot \kuka.

%This gives the system model of the Extended Kalman filter with to
The system model of the extended Kalman filter (EKF) can be written in the state-space form
\begin{subequations}\label{eq:dyn_sys_kalman_filter}
	\begin{align}
	\dot{\vec{z}} &= \vec{f}\left(\vec{z},\vec{u},\vec{w}\right)=
    \begin{bmatrix}
	\frac{1}{2}\vec{\Omega}(\tilde{\bm{\omega}}_\csym^\osym-\vec{w}_\omega)\vec{r}_\csym^\osym\\
	-\tilde{\dot{\mathbf{p}}}_0^\csym+\vec{w}_v
	\end{bmatrix}
    %,\quad \vec{x}\left(0\right)=\vec{x}_0
    \Comma\\
	\vec{y} &= \vec{h}\left(\vec{z},\vec{v}\right) =\begin{bmatrix}
		\vec{r}_{\csym}^\osym\\
		\vec{p}_{\csym}^\osym
	\end{bmatrix}+\vec{v} \Comma
\end{align}
\end{subequations}
with the system state $\vec{z}^\mathrm{T}=[\braces{\vec{r}_\csym^\osym}^\mathrm{T}, \braces{\vec{p}_\csym^\osym}^\mathrm{T}]\in\mathbb{R}^7$, the system input $\vec{u}^\mathrm{T}=[(\tilde{\bm{\omega}}_\csym^\osym)^\mathrm{T},(\tilde{\dot{\vec{p}}}_\csym^\osym)^\mathrm{T}]^\mathrm{T}\in\mathbb{R}^6$, 
the stochastic process perturbation $\vec{w}^\mathrm{T}=[\transpose{\vec{w}_\omega}, 
\transpose{\vec{w}_v}]\in\mathbb{R}^6$, the system output $\vec{y}^\mathrm{T}=[\transpose{\braces{\vec{r}_c^o}}, \transpose{\braces{\vec{d}_c^o}}]\in\mathbb{R}^7$, and the stochastic measurement noise $\vec{v}\in\mathbb{R}^7$. Since the EKF is implemented in a digital computer with the sampling time $T_a$, (\ref{eq:dyn_sys_kalman_filter}) is discretized by using Euler's method, resulting in 
%The Extended Kalman filter is implemented on a digital computer with sampling time $T_a$. Assuming a small sampling time and that between two sampling times $kT_a\leq t < \left(k+1\right)T_a$ the input variables are constant with $\vec{u}(t)=\vec{u}(kT_a)=\vec{u}_k$, (\ref{eq:dyn_sys_kalman_filter}) and Euler's method yield the nonlinear sampling system
\begin{subequations}
	\begin{align}\label{eq:kalman-filter_abtastsystem_sysdyn}
		\vec{z}_{k+1}&= \vec{F}\left(\vec{z}_k,\vec{u}_k, \vec{w}_k\right) =\vec{z}_{k} + \vec{f}\left(\vec{z}_k,\vec{u}_k, \vec{w}_k\right)T_a \Comma
            %, \quad \vec{x}\left(0\right)=\vec{x}_0
            \\
		\label{eq:kalman-filter_abtastsystem_ausgang}
		\vec{y}_k &= \vec{h}\left(\vec{z}_k, \vec{v}_k\right)\FullStop
	\end{align}
\label{eq:kalman-filter_abtastsystem} 
\end{subequations}
Considering the prior $\hat{\vec{z}}_k^-$ and posterior $\hat{\vec{z}}_k^+$ estimation of the system state with the stochastic process perturbation $\mathbf{w}_k=0$, the EKF system model (\ref{eq:kalman-filter_abtastsystem_sysdyn}) and (\ref{eq:kalman-filter_abtastsystem_ausgang}) is linearized around $\hat{\vec{z}}_k^+$ and $\hat{\vec{z}}_k^-$ resulting in the form
\begin{subequations}\label{eq:kalman-filter_lin_abtastsystem}
	\begin{align}\label{eq:kalman-filter_lin_abtastsystem_sysdyn}
		\vec{z}_{k+1}&= \vec{\Phi}_k(\vec{z}_{k}-\hat{\vec{z}}_k^+) + \vec{F}\left(\hat{\vec{x}}_k^+,\vec{u}_k, \vec{0}\right)  + \vec{G}_k\vec{w}_k\\
		\label{eq:kalman-filter_lin_abtastsystem_ausgang}
		\vec{y}_k &= \vec{C}_k(\vec{z}_k-\hat{\vec{z}}_k^-) + \vec{h}\left(\hat{\vec{x}}_k^-, \vec{0}\right) - \vec{C}_k + \vec{v}_k \Comma
	\end{align}
\end{subequations}
with
\begin{subequations}\label{eq:kalman-filter_part_diff}
	\begin{align}
		\vec{\Phi}_k& = \left.\PartDiff{\vec{F}\left(\vec{z}_k,\vec{u}_k, \vec{w}_k\right)}{\vec{z}_k}\right\rvert_{\vec{z}_k = \hat{\vec{x}}_k^+, \vec{u}_k = \vec{u}_k, \vec{w}_k=\vec{0}}
 \\
		\vec{C}_k &=  \left.\PartDiff{\vec{h}\left(\vec{z}_k,\vec{w}_k\right)}{\vec{z}_k}\right\rvert_{\vec{z}_k = \hat{\vec{z}}_k^-, \vec{w}_k=\vec{0}}
	\end{align}
\end{subequations}
%and the error covariance matrix $\vec{P}_k^-$, the a and the error covariance matrix $\vec{P}_k^+$
%To derive the iteration equations for the Extended Kalman filter, first a Taylor series expansion for the right-hand side of the system dynamics (\ref{eq: kalman-filter_sampling_system_sysdyn}) a Taylor series expansion around the point $\vec{x}_k=\hat{\vec{x}}_k^+$, $\vec{u}_k=\vec{u}_k$ and $\vec{w}_k=\vec{0}$, and for the right-hand side of the output equation (\ref{eq: kalman-filter_sampling_output}) a Taylor series expansion around the point $\vec{x}_k=\hat{\vec{x}}_k^-$ and $\vec{v}_k=\vec{0}$, and terminated after the linear term in each case. 
\iffalse
This results in the linearized sampling system
\begin{subequations}\label{eq:kalman-filter_lin_abtastsystem}
	\begin{align}\label{eq:kalman-filter_lin_abtastsystem_sysdyn}
		\vec{x}_{k+1}&= \vec{\Phi}_k\vec{x}_{k} + \bar{\vec{u}}_k + \vec{G}_k\vec{w}_k\\
		\label{eq:kalman-filter_lin_abtastsystem_ausgang}
		\vec{y}_k &= \vec{C}_k\vec{x}_k + \breve{\vec{u}}_k + \vec{v}_k.
	\end{align}
\end{subequations}
with the system matrices $\vec{\Phi}_k\in \mathbb{R}^{7\times7}$, $\vec{G}_k\in \mathbb{R}^{7\times6}$ and $\vec{C}_k\in \mathbb{R}^{7\times7}$,  the $n\times n$ unit matrix $\vec{E}_{n\times n}$ and the vectors $\bar{\vec{u}}_k\in \mathbb{R}^7$ and $\breve{\vec{u}}_k\in \mathbb{R}^7$ according to 
\begin{subequations}\label{eq:kalman-filter_part_diff}
	\begin{align}
		\vec{\Phi}_k& = \PartDiff{\vec{F}\left(\hat{\vec{x}}_k^+,\vec{u}_k, \vec{0}\right)}{\vec{x}_k}=
        \begin{bmatrix}
			\vec{E}_{4\times4}+\frac{1}{2}T_a\vec{\Omega}(\vec{u}_{k,1:3}) & \vec{0}_{4\times 3}\\
			\vec{0}_{3\times 4} & \vec{E}_{3\times3}
		\end{bmatrix}, \\
		\vec{G}_k &= \PartDiff{\vec{F}\left(\hat{\vec{x}}_k^+,\vec{u}_k, \vec{0}\right)}{\vec{w}_k} 
                %= 
                %\frac{T_a}{2}\begin{bmatrix}
			%-\hat{\vec{x}}_{k,2}^+ & -\hat{\vec{x}}_{k,3}^+ & -\hat{\vec{x}}_{k,4}^+ & 0 & 0 & 0 \\
			%\hat{\vec{x}}_{k,1}^+ & -\hat{\vec{x}}_{k,4}^+ & \hat{\vec{x}}_{k,3}^+ & 0 & 0 & 0\\
			%\hat{\vec{x}}_{k,4}^+ & \hat{\vec{x}}_{k,1}^+ & -\hat{\vec{x}}_{k,2}^+ & 0 & 0 & 0\\
			%-\hat{\vec{x}}_{k,3}^+ & \hat{\vec{x}}_{k,2}^+ & \hat{\vec{x}}_{k,1}^+ & 0 & 0 & 0\\
			%0 & 0 & 0 & 2 & 0 & 0\\		
			%0 & 0 & 0 & 0 & 2 & 0\\		
			%0 & 0 & 0 & 0 & 0 & 2\\		
		%\end{bmatrix},\\
		\vec{C}_k &= \PartDiff{\vec{h}\left(\hat{\vec{x}}_k^-, \vec{0}\right)}{\vec{x}_k} = \vec{E}_{7\times7},\\
		\bar{\vec{u}}_k &= \vec{F}\left(\hat{\vec{x}}_k^+,\vec{u}_k, \vec{0}\right) - \vec{\Phi}_k\hat{\vec{x}}_k^+,\\
		\breve{\vec{u}}_k &= \vec{h}\left(\hat{\vec{x}}_k^-, \vec{0}\right) - \vec{C}_k\hat{\vec{x}}_k^-.
	\end{align}
\end{subequations}

Here $\vec{x}_{k,i}$ or $\vec{u}_{k,i}$ denotes the $i$th element of the state $\vec{x}_k$ or the input $\vec{u}_k$, respectively. For the partial derivatives in (\ref{eq:kalman-filter_part_diff}) the simplified notation applies in each case
\begin{equation}
	\PartDiff{\vec{F}\left(\hat{\vec{x}}_k^+,\vec{u}_k, \vec{0}\right)}{\vec{x}_k} = \left.\PartDiff{\vec{F}\left(\vec{x}_k,\vec{u}_k, \vec{w}_k\right)}{\vec{x}_k}\right\rvert_{\vec{x}_k = \hat{\vec{x}}_k^+, \vec{u}_k = \vec{u}_k, \vec{w}_k=\vec{0}}
\end{equation}

Furthermore, for the disturbance $\vec{w}_k$ and the measurement noise $\vec{v}_k$ it is assumed that with the Kronecker symbol $\delta_{kj}=1$ for $k=j$ and $\delta_{kj}=0$ holds otherwise
\begin{subequations}
	\begin{align}
		\text{E}\left(\vec{v}_k\right) &= \vec{0} & \text{E}\left(\vec{v}_k\transpose{\vec{v}_j}\right)&=\vec{R}_k\delta_{kj}\\
		\text{E}\left(\vec{w}_k\right) &= \vec{0} & \text{E}\left(\vec{w}_k\transpose{\vec{w}_j}\right)&=\vec{Q}_k\delta_{kj}\\
		& & \text{E}\left(\vec{w}_k\transpose{\vec{v}_j}\right)&=\vec{0}.
	\end{align}
\end{subequations}
The values of $\vec{R}_k$ and $\vec{Q}_k$ are given in table \ref{tab:kalman_filter_matrizes} in the Appendix.

The measured output $\vec{y}_k$ is the pose $\left[\vec{R}_c^o|\vec{t}_c^o\right]$ calculated via the EP\textit{n}P algorithm from (\ref{eq:EPnP}), where the rotation matrix $\vec{R}_c^o$ is converted via (\ref{eq: quat_rotmat}) is converted to the quaternion $\vec{r}_c^o$, and the vector $\vec{t}_c^o$ in the camera coordinate system is transformed to the base coordinate system via $\vec{d}_c^o=\vec{R}_0^c\vec{t}_c^o$.
\fi
Here, the update rules of the EKF are defined by following the equations 
\begin{subequations}
	\begin{align}
		\hat{\vec{L}}_k &= \vec{P}_k^-\transpose{\vec{C}_k}\left(\vec{C}_k\vec{P}_k^-\transpose{\vec{C}_k}+\vec{R}_k\right)^{-1}\\
		\label{eq:x_extrapolation}
		\hat{\vec{z}}_k^+ &= \hat{\vec{z}}_k^- + \hat{\vec{L}}_k \left(\vec{y}_k-\vec{C}_k\hat{\vec{z}}_k^-\right)\\
		\label{eq:P_extrapolation}
		\vec{P}_k^+ &= \left(\vec{I}_{7}-\hat{\vec{L}}_k\vec{C}_k\right)\vec{P}_k^- \\
		%\vec{\Phi}_k& = \PartDiff{\vec{F}\left(\hat{\vec{x}}_k^+,\vec{u}_k, \vec{0}\right)}{\vec{x}_k} \\
		%\vec{G}_k &= \PartDiff{\vec{F}\left(\hat{\vec{x}}_k^+,\vec{u}_k, \vec{0}\right)}{\vec{w}_k} \\
		\hat{\vec{z}}_{k+1}^- &= \vec{F}\left(\hat{\vec{z}}_k^+,\vec{u}_k, \vec{0}\right) \\ 
		\vec{P}_{k+1}^- &= \vec{\Phi}_k \vec{P}_k^+ \transpose{\vec{\Phi}_k} + \vec{G}_k\vec{Q}_k\transpose{\vec{G}_k} \Comma
	\end{align}
 \label{eq: EKF update}
\end{subequations}
where $\hat{\vec{z}}_k^-$ and $\hat{\vec{z}}_k^+$ are the prior and posterior estimated EKF system state, respectively, $\vec{P}_k^-$ and $\vec{P}_k^+$ are the prior and posterior covariance matrix, respectively, $\hat{\vec{L}}_k$ is the Kalman gain matrix, and $\vec{I}_{7}$ is the identity matrix with the size $7$. Additionally, $\mathbf{R}_k$ and $\mathbf{Q}_k$ are the user-defined diagonal matrices. %For more information on the implementation of the EKF, readers are referred to \cite{Koenigseder17}.

Since the sampling rate of the camera is longer than the sampling time $T_a$ of the EKF, the computations of (\ref{eq:x_extrapolation}) and (\ref{eq:P_extrapolation}) are only taken when a new measurement $\vec{y}_k$ from (\ref{eq:EPnP}) is available. Here, the EKF yields the estimated translation $\hat{\vec{p}}_\csym^\osym$ and the estimated quaternion $\hat{\mathbf{r}}_\csym^\osym$ which can be transformed into rotation matrix $\hat{\mathbf{R}}_\csym^\osym$ \cite{shepperd1978quaternion}. Thereby, the estimated pose of the object in the world coordinate system is given by
\begin{equation}
    \begin{aligned} 
    	\hat{\vec{H}}_0^\osym &=
        \begin{bmatrix}
    		\vec{R}_0^\csym\hat{\vec{R}}_\csym^\osym & \vec{p}_0^\csym+\vec{R}_0^\csym\hat{\vec{p}}_\csym^\osym \\
    		\transpose{\vec{0}} & 1
    	\end{bmatrix} = 
        \begin{bmatrix}
    		\hat{\vec{R}}_0^\osym & \hat{\vec{p}}_0^\osym \\
    		\transpose{\vec{0}} & 1
    	\end{bmatrix} \FullStop
    \end{aligned}
\label{eq:homogene_transformation_objekt_estimated} 
 \end{equation}

%Using the estimated pose (\ref{eq:homogene_transformation_objekt_estimated}) of the object, trajectory planning is performed in the next chapter. 
